See Without Decoding: Motion-Vector-Based Tracking in Compressed Video

We propose a lightweight compressed-domain tracking model that operates directly on video streams, without requiring full RGB video decoding. Using motion vectors and transform coefficients from compressed data, our deep model propagates object bounding boxes across frames, achieving a computational speed-up of order up to 3.7 with only a slight 4% mAP@0.5 drop vs RGB baseline on MOTS15/17/20 datasets. These results highlight codec-domain motion modeling efficiency for real-time analytics in large monitoring systems.

==> backup_schema.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.95\linewidth]{figs/motion_block_estimation}
\caption{Block motion estimation in MPEG-4: the encoder searches for matching blocks between consecutive frames, computing motion vectors $MV_n^g$ and residuals $\Delta Y_n^g$ (pixel subtraction). The search zone shows candidate blocks explored during estimation.}
\label{fig:motion_estimation}
\vspace{-0.4em}
\end{figure}
